Fingerprinting the Fingerprinters: Learning to Detect Browser Fingerprinting Behaviors

Browser fingerprinting is an invasive and opaque stateless tracking technique. Browser vendors, academics, and standards bodies have long struggled to provide meaningful protections against browser fingerprinting that are both accurate and do not degrade user experience. We propose FP-Inspector, a machine learning based syntactic-semantic approach to accurately detect browser fingerprinting. We show that FP-Inspector performs well, allowing us to detect 26% more fingerprinting scripts than the state-of-the-art. We show that an API-level fingerprinting countermeasure, built upon FP-Inspector, helps reduce website breakage by a factor of 2. We use FP-Inspector to perform a measurement study of browser fingerprinting on top-100K websites. We find that browser fingerprinting is now present on more than 10% of the top-100K websites and over a quarter of the top-10K websites. We also discover previously unreported uses of JavaScript APIs by fingerprinting scripts suggesting that they are looking to exploit APIs in new and unexpected ways.

==> Makefile <==
extensions_to_clean := out aux log bbl blg fls fdb_latexmk glg gls lof glo glsdefs lot toc dvi ist acn acr synctex.gz alg xdy

all: paper

clean:
	@if [[ -f paper.pdf ]]; then \
		rm paper.pdf;\
	fi;
	@for extension in $(extensions_to_clean); do \
		find . -type f -name "*.$$extension" -delete;\
	done;

paper:
	latexmk -bibtex -pdf paper
	pdflatex -bibtex -interaction=nonstopmode paper

==> docs/dynamic_features_info_gain <==
=== Run information ===

Evaluator:    weka.attributeSelection.InfoGainAttributeEval 
Search:       weka.attributeSelection.Ranker -T -1.7976931348623157E308 -N -1
Relation:     features_with_encoding-weka.filters.unsupervised.attribute.RemoveType-Tstring-weka.filters.unsupervised.attribute.PartitionedMultiFilter-Fweka.filters.supervised.attribute.AttributeSelection -E "weka.attributeSelection.InfoGainAttributeEval " -S "weka.attributeSelection.Ranker -T -1.7976931348623157E308 -N 1000"-R3-last-weka.filters.unsupervised.attribute.Reorder-R1002,1003,first-1001-weka.filters.unsupervised.attribute.RenameAttribute-find^(filtered-0-|unfiltered-)(\w+)+$-replace$2-Rfirst-last-weka.filters.unsupervised.attribute.RenameAttribute-find^(filtered-0-|unfiltered-)(\w+[\+]*\w+)+$-replace$2-Rfirst-last-weka.filters.unsupervised.attribute.Reorder-R2,1,3-last-weka.filters.unsupervised.attribute.Remove-R1-2
Instances:    153354
Attributes:   1001
              [list of attributes omitted]
Evaluation mode:    evaluate on all training data



=== Attribute Selection on all input data ===

Search Method:
	Attribute ranking.

Attribute Evaluator (supervised, Class (nominal): 1001 class):
	Information Gain Ranking Filter

Ranked attributes:
 0.03877192343       1 fog79
 0.03760103568       2 fog90
 0.03565229699       3 fog70
 0.03531607851       4 fog80
 0.03365408991       5 fog88
 0.03300298329       6 fvcu3_2+0
 0.03266744005       8 fog68
 0.03230486754       7 fog89
 0.02892051979       9 fog49
 0.02466484136      11 fog34
 0.02452592428      10 fog71
 0.02263690604      12 fvcu3_1+0
 0.0222958398       14 fog54
 0.02194866693      13 fvcu3_3+0
 0.02172286498      15 fog23
 0.0216995108       16 fog114
 0.02151392683      17 fog113
 0.02027182272      18 fog74
 0.01956471486      19 fvca1_1+0
 0.01875964514      20 fog52
 0.01870628094      24 fog119
 0.0186469379       21 fog77
 0.01854607459      23 fog78
 0.01853135414      25 fog116
 0.0185211047       26 fog122
 0.0185211047       27 fog123
 0.01852068624      22 fog93
 0.01839572867      28 fog121
 0.01834305962      32 fog120
 0.01818563525      31 fog33
 0.01816375555      33 fog111
 0.01800291408      36 fog107
 0.01794184786      40 faca30_1+1
 0.01791397489      29 fog94
 0.01789805831      30 fog95
 0.01789705063      35 fog21
 0.01784873536      34 fog92
 0.01783117349      38 fog109
 0.01783031665      41 fog106
 0.0178153779       39 fog97
 0.01778709239      42 fog105
 0.01776823876      43 fog108
 0.01773743656      45 fog118
 0.01773171247      46 faca30_2+0
 0.01766537262      49 fog115
 0.01766327953      47 fog98
 0.01756510474      50 fog96
 0.01752244146      52 fog87
 0.01750215593      51 fcu80_1+0
 0.01749448751      37 fvcu3_4+0
 0.01747123547      54 fog117
 0.01743129819      53 fcu24_1+0
 0.01743004709      55 faca30_3+0
 0.01737599378      56 fog99
 0.01737599378      57 fog104
 0.01737599378      58 fog103
 0.0173618099       59 fog102
 0.0173618099       60 fog101
 0.0173618099       61 fog100
 0.01733316172      44 fvcu3_5+0
 0.01725377834      48 fog91
 0.01723165148      62 fcu152_1+0
 0.0171588176       63 fcu2_1+0
 0.01712787658      64 fcu57_1+0
 0.0170913593       65 fog85
 0.01703888629      66 fog86
 0.01699831946      68 fcu69_1+0
 0.01699831946      67 fcu42_1+0
 0.01683020102      69 fog110
 0.01628485502      70 fog112
 0.01525004547      71 fvca6_1+0
 0.01401364349      72 fog47
 0.01334196048      74 fog35
 0.01332805449      73 fog72
 0.01308959237      78 faca30_4+0
 0.01304947706      75 fog48
 0.01294183557      76 fog57
 0.01292692895      77 fog6
 0.0125191217       79 fog55
 0.01247169493      80 fog56
 0.01223925765      81 fog10
 0.01178280182      82 fog15
 0.01156480108      83 fog20
 0.01129079517      85 fog73
 0.01127216608      84 fog13
 0.00987017128      87 fog17
 0.00977513678      88 fog45
 0.0096404019       89 fog82
 0.00960741106      86 fvcu3_4+1
 0.00954055354      90 fog163
 0.00950116136      91 fog200
 0.00932119896      93 fvcu3_1+1
 0.00931583667      94 fog81
 0.00925232873      92 fvcu3_3+1
 0.00912530856      95 fvca1_1+1
 0.00862171781      97 fog139
 0.00862171781      96 fog133
 0.00856368797      98 fog132
 0.00842968105      99 fog141
 0.00830466592     100 fog32
 0.0081534663      101 fog2
 0.00762822758     104 fog24
 0.00762409847     102 fog153
 0.00762409847     103 fog154
 0.00762054917     108 fog83
 0.0075743457      105 fog155
 0.00756720127     107 fog152
 0.00756720127     106 fog149
 0.00753123572     109 fvca1_2+0
 0.00702126972     110 fvca17_1+0
 0.00682312132     111 fog150
 0.00639737649     112 fog37
 0.00618612178     113 fog151
 0.00577270312     115 fcu154_1
 0.00575441213     114 faca30_5+0
 0.00551884609     116 fcu154_2
 0.00465981974     117 fog156
 0.003725181       118 fvj1_2
 0.00369067968     119 fvca6_3+0
 0.00336413505     120 fog38
 0.00297858394     121 fvj1_5
 0.00289986228     122 fcu80_2+0
 0.00281494572     123 fcu152_2+0
 0.00278207198     124 fcu57_2+0
 0.00277040412     125 fcu24_2+0
 0.00270426535     126 fog195
 0.00264259074     127 fvca6_2+0
 0.00245564486     128 fvca6_2+1
 0.00244826388     129 fvca1_3+1
 0.00243955641     130 fvca6_1+1
 0.00222062399     132 fcu42_2+0
 0.00222062399     131 fcu69_2+0
 0.00212684678     133 faca30_3+3
 0.00202665292     135 fog40
 0.00195134969     137 fog140
 0.00193416813     134 fcu2_2+0
 0.00191881037     136 fog19
 0.00187560632     141 fog7
 0.00187483778     139 fcu80_3+0
 0.00186689674     138 fog3
 0.00183734757     140 faca30_4+2
 0.00178646636     142 fcu152_3+0
 0.00176921098     143 fcu57_3+0
 0.00175694402     144 faca30_2+3
 0.00167552036     145 fog136
 0.00167505481     146 faca30_1+0
 0.00164690613     147 fog215
 0.00164651403     148 fcu24_3+0
 0.00159326718     149 fvca1_4+0
 0.00149410013     150 fvca17_1+1
 0.0014574265      152 fog16
 0.00143762598     151 fog201
 0.00142840251     153 fcu80_4+0
 0.00136960065     156 fog36
 0.00134023556     157 fcu2_4+0
 0.0013381712      155 fog179
 0.00133085345     159 fcu57_4+0
 0.00133085345     158 fcu152_4+0
 0.00131379193     154 faca44_1+2
 0.00130821155     160 fog128
 0.00130075784     163 fog292
 0.00130075784     164 fog291
 0.00130075784     162 fog294
 0.00130075784     165 fog293
 0.00130075784     161 fog295
 0.00128313598     166 fog335
 0.00120031099     167 fcu80_5+0
 0.00112049997     168 fcu57_5+0
 0.00111648483     177 fog26
 0.00111424708     169 fcu152_5+0
 0.00110758144     170 fcu42_3+1
 0.00110758144     173 fcu69_3+1
 0.00110758144     172 fog135
 0.00110758144     171 fog138
 0.00109108716     174 fog229
 0.00107985708     175 fog25
 0.00105931318     176 fog290
 0.00103490432     178 fog234
 0.00102851803     193 fog0
 0.00102067141     179 fog134
 0.00101775345     195 fcu165_1
 0.00101681343     180 fog208
 0.00101139048     181 fog301
 0.00101122285     182 fog289
 0.00101105523     191 fcu69_2+2
 0.00101105523     186 fcu69_1+3
 0.00101105523     189 fog302
 0.00101105523     190 fcu42_2+2
 0.00101105523     184 fcu42_3+2
 0.00101105523     188 fcu42_4+2
 0.00101105523     187 fcu42_1+3
 0.00101105523     185 fcu69_3+2
 0.00101105523     183 fcu42_5+2
 0.00098584211     192 fog130
 0.00097946905     194 fog207
 0.00097468537     196 fog230
 0.00096264728     206 fog243
 0.00095688212     217 fog53
 0.00094151789     197 fog233
 0.00092955873     198 fog210
 0.00092811536     199 fcu2_3+1
 0.00092671345     200 fog235
 0.0009145702      204 fog296
 0.0009145702      205 fog297
 0.0009145702      202 fog298
 0.0009145702      203 fog299
 0.0009145702      201 fog300
 0.00090253421     207 fog127
 0.0008982188      208 fog209
 0.00089479049     209 fog131
 0.00089193484     210 fog240
 0.00088366147     212 fog206
 0.00088261664     213 fog137
 0.00086938409     214 fog148
 0.00086634312     215 faca30_5+2
 0.00085270252     211 fvcu4_1+1
 0.00085226305     216 fog239
 0.00084404599     218 fog220
 0.00083915487     219 fcu2_3+0
 0.00082954345     220 faca30_4+3
 0.00082928489     221 fcu2_2+1
 0.00082313815     222 fog129
 0.00076991972     223 fog242
 0.00076619669     224 fcu123_1+0
 0.00074966612     225 fcu2_5+1
 0.00072172339     229 fcu69_4+1
 0.00072172339     227 fvca6_4+0
 0.00072172339     228 fcu42_4+1
 0.00070682326     226 fvcu3_5+1
 0.00070314427     230 fog22
 0.00068858051     232 fog59
 0.00063868214     234 fog5
 0.00063730166     231 fcu154_3
 0.00060333151     233 fvj1_1
 0.00060029024     243 fog190
 0.00059267936     236 fvj2_1
 0.00059152723     235 faca30_5+3
 0.00058017695     242 fog18
 0.00057403209     237 fog9
 0.00057080219     239 fvca1_5+1
 0.00056408846     241 fvj1_4
 0.00056135667     253 fog180
 0.00055724256     240 faca44_5+2
 0.00055355655     238 fog262
 0.00053798323     248 fog29
 0.00052904029     245 fcu42_5+1
 0.00052904029     246 fcu69_5+1
 0.00052735649     247 fog65
 0.00051463639     250 fcu154_4
 0.00051143581     251 fvca1_3+0
 0.00050881227     252 fcu24_4+0
 0.00050391556     244 fvcu3_2+1
 0.00049935775     249 fvca1_2+1
 0.00049772942     255 fog14
 0.00049405052     254 fog192
 0.00049393787     256 fog191
 0.00047892829     257 fog258
 0.00047705392     259 faca44_3+1
 0.0004766475      258 fvca6_5+0
 0.00046999039     260 fvca1_5+0
 0.00046012642     262 fvcu1_1+1
 0.00041578738     261 faca44_4+2
 0.00040106022     263 fcu2_5+0
 0.00039323275     264 fog27
 0.00038463495     271 fog43
 0.00038463495     265 faca30_3+9
 0.00037686426     266 fog259
 0.0003740589      267 fog126
 0.00036095541     268 fog60
 0.00035928512     269 fcu24_5+0
 0.00035515653     270 faca30_5+8
 0.00034399641     272 fog162
 0.00033903953     273 faca44_2+1
 0.00032017827     274 fcu11_1
 0.00031762684     275 faca30_2+1
 0.0003038741      276 fcu11_2
 0.00030361219     277 fcu11_3
 0.00029717905     278 fcu11_4
 0.0002946401      279 fcu11_5
 0.00028841552     280 fvca13_1+1
 0.00028114154     281 fvca21_1+2
 0.00028075458     282 faca30_4+5
 0.00025280169     283 fog147
 0.00025224817     284 fvj1_3
 0.00024555362     285 fcu165_2
 0.00021579186     286 fcu165_3
 0.00019776852     287 fvca1_4+1
 0.0001922366      299 faca30_2+4
 0.0001922366      288 fvca13_2+1
 0.00018260206     289 fog76
 0.00017300063     290 fog166
 0.00016758096     292 fog187
 0.0001611191      293 faca44_4+1
 0.00014658755     294 fog8
 0.00014486917     295 fvj2_2
 0.00014416232     297 fvca13_3+1
 0.00014416232     296 fog402
 0.00014302832     298 faca44_5+1
 0.00013237544     311 fog275
 0.0001308402      343 fog193
 0.00012605644     300 fcu150_1
 0.00011394231     302 fcu150_2
 0.00011289106     301 fog84
 0.00011261911     326 fog251
 0.00011261911     327 fog204
 0.00011261911     312 fog257
 0.00011261911     329 fog252
 0.00010986945     303 fog196
 0.00010941011     304 faca37_1
 0.0001052081      322 fog254
 0.00010428875     315 fog182
 0.00010174735     316 fvcu1_2+1
 0.00009609813     307 fcu42_1+10
 0.00009609813     306 fcu42_2+9
 0.00009609813     305 fcu69_2+8
 0.00009061149     309 fcu69_1+2
 0.00008852472     308 fvcu2_3
 0.00008420675     334 fvcu1_5+1
 0.00008389372     310 fog11
 0.00008378146     314 fog31
 0.00008200439     392 fvj3_2
 0.00007922747     341 fvcu1_4+1
 0.00007922747     342 fvcu1_3+1
 0.00007819093     313 fog255
 0.00007337631     323 faca37_2
 0.00007145991     317 fog30
 0.00007043308     318 fog62
 0.00007012877     319 fog253
 0.00007012877     320 fvca6_5+1
 0.00007012877     321 fog256
 0.00006598683     325 fog223
 0.0000657751      324 fcu118_1
 0.00006538617     331 fcu3_1
 0.00006461209     328 fog264
 0.00006397505     330 fvcu4_1+0
 0.00005716894     338 fvj3_1
 0.00005698532     332 fog385
 0.00005684429     333 fcu61_1
 0.00005473146     336 faca17_3
 0.00005411853     335 fvca6_4+1
 0.00005313248     337 fvca5_4+2
 0.00005182543     340 fvca5_3+2
 0.00005164799     339 fog205
 0.00005129698     385 faca44_1+1
 0.00005048623     345 faca37_4
 0.00004804403     372 fog447
 0.00004804403     373 fcu42_3+10
 0.00004804403     370 fcu42_2+25
 0.00004804403     371 faca30_3+4
 0.00004804403     365 fog439
 0.00004804403     374 faca30_1+9
 0.00004804403     368 fcu69_3+20
 0.00004804403     367 fcu42_1+2
 0.00004804403     369 fvca13_1+2
 0.00004804403     377 fog279
 0.00004804403     375 fcu69_2+16
 0.00004804403     382 faca3_2+2
 0.00004804403     384 fcu42_5+30
 0.00004804403     383 faca3_4+1
 0.00004804403     381 fcu69_1+13
 0.00004804403     378 fog280
 0.00004804403     380 fcu69_2+23
 0.00004804403     379 fcu2_1+2
 0.00004804403     366 fcu42_3+29
 0.00004804403     376 fcu69_1+16
 0.00004804403     364 fog438
 0.00004804403     352 fog334
 0.00004804403     353 fcu42_4+30
 0.00004804403     363 fog437
 0.00004804403     351 fog408
 0.00004804403     350 fvca1_2+5
 0.00004804403     349 fvca1_1+5
 0.00004804403     347 fog440
 0.00004804403     346 fcu69_4+7
 0.00004804403     354 fcu42_5+11
 0.00004804403     348 fvca1_1+6
 0.00004804403     355 fcu42_1+27
 0.00004804403     360 fcu42_4+12
 0.00004804403     361 fcu69_5+19
 0.00004804403     356 fog398
 0.00004804403     359 fvca1_2+6
 0.00004804403     362 fvca13_2+2
 0.00004804403     358 fcu69_4+20
 0.00004804403     357 fcu42_2+17
 0.00004758782     386 fvcu4_2+0
 0.000047252       389 faca37_3
 0.00004659369     344 faca17_1
 0.00004580409     388 fcu2_4+1
 0.00004377596     391 fcu170_3
 0.00004283843     393 fcu170_4
 0.00004236334     395 faca46_1
 0.00004115454     396 fvca21_2+0
 0.00003788622     400 fcu139_1
 0.00003788622     399 fcu151_1
 0.0000375531      397 fcu154_5
 0.00003739043     398 fvca5_5+1
 0.00003505941     405 fog414
 0.00003505941     402 faca3_3+0
 0.00003505941     404 fcu69_3+9
 0.00003505941     403 faca3_3+1
 0.00003505941     401 faca3_2+0
 0.00003443969     390 faca44_3+2
 0.00003376227     406 faca46_2
 0.0000320992      407 fvj2_4
 0.00003170451     408 faca46_3
 0.00003050658     413 fcu117_1
 0.00003009896     410 fvcu4_4+0
 0.00002977483     409 fvj3_3
 0.00002975036     411 fvn37_3
 0.00002957719     412 faca17_2
 0.00002850152     414 fvcu4_3+0
 0.0000282151      422 faca37_5
 0.00002764984     417 fcu17_1
 0.00002688753     416 fvca7_1+2
 0.00002617293     415 fvcu2_5
 0.00002603513     419 fcu157_1
 0.00002584859     421 fcu128_1
 0.00002579057     420 fvj2_3
 0.00002487281     424 fcu157_2
 0.00002444039     423 fvca21_5+2
 0.00002399556     425 fvca21_4+2
 0.00002314436     426 fvca21_3+2
 0.00002202804     428 fcu100_4
 0.00002177974     429 fvn37_5
 0.00002140418     430 fcu17_2
 0.00002023153     427 fvca5_2+1
 0.00001937432     432 fvn37_4
 0.00001913846     433 fcu100_3
 0.00001817246     434 fcu41_2
 0.00001745994     456 fal4_1
 0.00001723358     436 fcu157_3
 0.00001708083     435 fal4_4
 0.00001676075     466 fal4_2
 0.0000165234      437 fcu140_1
 0.00001555554     439 fcu147_1
 0.00001509333     440 fvn37_2
 0.00001503042     438 fvca11_1
 0.00001444839     442 fal4_3
 0.00001431128     444 fcu41_1
 0.00001412334     443 fal4_5
 0.0000134197      441 fcu165_5
 0.00001319706     446 fcu34_2
 0.00001266852     447 fcu150_3
 0.00001217934     448 fcu150_4
 0.00001202        449 fvj2_5
 0.00001197725     445 fcu165_4
 0.00001128425     451 fcu169_2
 0.00001128425     450 fcu110_2
 0.0000108451      452 fcu127_5
 0.00001068188     453 fcu127_2
 0.00001016571     454 fcu29_1
 0.00000999873     455 fcu110_1
 0.00000985614     464 fcu170_5
 0.00000963708     457 faca26_1
 0.00000947965     460 fcu34_3
 0.00000939533     458 fcu3_2
 0.00000924458     459 fcu127_4
 0.00000919327     461 fcu127_3
 0.00000878293     462 fvn17_1
 0.0000085139      465 fvl5_1
 0.00000839652     463 fcu140_2
 0.00000776342     467 fcu161_1
 0.00000773071     469 fcu33_1
 0.00000769565     470 faca14_2
 0.00000761353     468 fvn37_1
 0.00000756504     471 fcu169_3
 0.00000738235     472 faca28_2
 0.00000668597     473 fcu61_2
 0.00000642437     474 fvl5_2
 0.00000635087     475 fcu127_1
 0.00000634173     476 faca28_1
 0.00000580393     477 fcu150_5
 0.00000575732     478 faca14_3
 0.00000570905     479 fcu110_3
 0.00000519552     480 fvj6_5
 0.00000516926     481 fcu117_2
 0.0000046631      482 fcu140_3
 0.00000465974     483 fcu128_2
 0.00000458324     484 fcu61_3
 0.00000450534     486 faca17_5
 0.00000450534     485 faca17_4
 0.0000044742      487 fcu26_2
 0.00000420545     490 fcu86_2
 0.00000384958     493 fcu146_1
 0.00000379419     492 fcu139_2
 0.00000379419     491 fcu151_2
 0.00000367841     494 fcu3_4
 0.00000326441     495 fcu117_3
 0.00000304698     496 fcu3_5
 0.00000289869     497 faca46_4
 0.00000288328     498 faca28_3
 0.00000281711     499 faca46_5
 0.00000270681     501 fcu161_2
 0.00000247928     502 fcu128_3
 0.00000224288     503 faca28_4
 0.00000221217     533 faca32_3
 0.00000219164     504 fcu161_3
 0.0000021762      505 fcu17_3
 0.0000021762      506 fcu86_3
 0.00000209032     507 fcu157_5
 0.00000202643     508 fvn36_1
 0.00000183571     500 fal2_1
 0.00000177179     509 fcu33_2
 0.0000017044      510 faca26_2
 0.00000164813     512 fcu79_1
 0.00000164813     511 fcu79_2
 0.00000160913     513 fcu157_4
 0.00000159575     514 fcu151_3
 0.00000159575     515 fcu139_3
 0.00000150298     516 fcu61_4
 0.00000149746     517 fcu147_2
 0.00000149234     549 faca32_2
 0.0000014852      537 faca32_4
 0.00000144806     518 fcu26_1
 0.00000141774     519 faca33_1
 0.00000128529     520 faca26_3
 0.00000126945     521 fcu41_4
 0.00000123121     522 fcu128_4
 0.00000120276     524 fcu3_3
 0.00000120276     523 fcu33_3
 0.00000118331     525 fcu118_2
 0.00000110827     526 fcu128_5
 0.00000106817     527 faca14_4
 0.00000106817     528 faca14_5
 0.00000106076     530 fcu139_4
 0.00000106076     529 fcu151_4
 0.00000105919     531 faca28_5
 0.000001057       532 fvn24_1
 0.00000098863     534 fcu61_5
 0.00000095181     536 fcu34_5
 0.00000095181     535 fcu34_4
 0.00000079443     538 fcu139_5
 0.00000079443     539 fcu151_5
 0.00000078931     832 faca32_1
 0.00000074809     543 fcu110_5
 0.00000074809     542 fcu169_4
 0.00000074809     540 fcu110_4
 0.00000074809     541 fcu169_5
 0.00000074705     544 fcu117_4
 0.00000073116     545 fcu146_2
 0.000000699       546 fcu19_1
 0.00000068249     548 faca38_2
 0.00000068249     547 faca38_3
 0.00000062796     550 faca26_4
 0.00000060191     551 fcu41_3
 0.0000005638      553 fcu51_1
 0.0000005638      552 fcu102_1
 0.00000055988     625 fvn5_5
 0.00000051098     554 fcu117_5
 0.00000049902     621 fcu142_1
 0.0000004491      556 fcu147_3
 0.00000042368     557 fcu146_3
 0.00000034841     558 faca41_2
 0.00000034011     559 fcu33_5
 0.00000032941     827 faca32_5
 0.00000030851     561 fvn5_1
 0.00000028794     560 fcu41_5
 0.00000014485     591 fcu111_2
 0.00000014485     581 fcu111_3
 0.00000013725     562 fvn24_2
 0.00000007463     623 fcu134_1
 0.00000004072     568 fcu102_2
 0.00000004072     567 fcu51_2
 0.00000001527     569 fcu51_3
 0.00000001527     570 fcu102_3
 0.00000001018     572 fcu102_4
 0.00000001018     573 fvn15_1
 0.00000001018     571 fcu51_4
 0.00000000509     575 fvn15_2
 0.00000000509     574 fcu160_2
 0.00000000509     576 fcu160_3
 0                 853 fvca2_1
 0                 852 fcu161_4
 0                 840 fcu27_5
 0                 855 fcu158_3
 0                 851 fcu107_4
 0                 854 fcu158_1
 0                 858 fcu19_2
 0                 856 fcu158_4
 0                 859 fcu19_3
 0                 850 fcu37_2
 0                 857 fcu158_5
 0                 887 faca12_3
 0                 888 faca12_1
 0                 849 fcu37_1
 0                 843 fcu37_4
 0                 841 fcu7_1
 0                 889 fcu161_5
 0                 890 fcu74_3
 0                 842 fcu27_1
 0                 844 fcu79_5
 0                 848 fcu26_5
 0                 845 fcu37_3
 0                 847 fcu26_4
 0                 860 fcu158_2
 0                 846 fcu26_3
 0                 886 faca11_2
 0                 864 faca12_4
 0                 861 fcu91_5
 0                 874 fcu132_2
 0                 878 fcu168_4
 0                 877 fcu132_5
 0                 876 fcu132_4
 0                 884 faca35_5
 0                 879 fcu168_2
 0                 880 faca35_2
 0                 883 faca35_4
 0                 882 faca35_3
 0                 881 fcu168_1
 0                 875 fcu132_3
 0                 873 fcu168_5
 0                 862 fcu19_5
 0                 872 fcu168_3
 0                 866 fcu91_1
 0                 865 faca12_5
 0                 863 fcu91_4
 0                 867 fcu91_2
 0                 868 fcu91_3
 0                 885 faca11_1
 0                 871 faca12_2
 0                 870 faca35_1
 0                 869 fcu19_4
 0                 999 fog347
 0                 809 fcu65_5
 0                 839 fcu27_4
 0                 804 fcu107_2
 0                 802 fcu77_5
 0                 801 fcu77_4
 0                 800 fcu77_2
 0                 803 fcu107_1
 0                 805 fcu107_3
 0                 838 fcu27_3
 0                 806 fcu77_3
 0                 892 fcu144_1
 0                 808 faca20_4
 0                 807 fcu77_1
 0                 799 fcu7_4
 0                 798 faca20_3
 0                 797 faca20_1
 0                 796 faca36_1
 0                 789 faca36_3
 0                 788 faca36_5
 0                 787 faca5_5
 0                 790 faca20_2
 0                 791 faca36_2
 0                 792 faca33_2
 0                 795 faca33_5
 0                 794 faca33_4
 0                 793 faca33_3
 0                 810 faca20_5
 0                 811 fcu65_1
 0                 812 fcu65_2
 0                 825 faca41_1
 0                 830 fcu147_4
 0                 829 fcu118_5
 0                 828 fcu118_4
 0                 831 fcu147_5
 0                 833 fcu122_5
 0                 834 fcu79_4
 0                 837 fcu27_2
 0                 836 fcu37_5
 0                 835 fcu7_2
 0                 826 fcu79_3
 0                 824 faca41_4
 0                 813 fcu65_3
 0                 823 fcu122_4
 0                 816 fcu7_3
 0                 815 fcu7_5
 0                 814 fcu65_4
 0                 817 fcu107_5
 0                 818 faca41_3
 0                 819 faca41_5
 0                 822 fcu122_3
 0                 821 fcu122_2
 0                 820 fcu122_1
 0                 891 fcu74_5
 0                 925 fcu72_4
 0                 893 fcu144_2
 0                 966 fog307
 0                 964 fog309
 0                 963 fog308
 0                 962 fog310
 0                 965 fog306
 0                 967 fog305
 0                 973 fog338
 0                 968 fog287
 0                 971 fog304
 0                 970 fog303
 0                 969 fog288
 0                 961 fog286
 0                 960 fog284
 0                 959 fog276
 0                 958 fog274
 0                 951 fog282
 0                 950 fog311
 0                 949 fog312
 0                 952 fog283
 0                 953 fog278
 0                 954 fog281
 0                 957 fog273
 0                 956 fog285
 0                 955 fog277
 0                 972 fog337
 0                 974 fog339
 0                 947 fog329
 0                 993 fog377
 0                 991 fog380
 0                 990 fog382
 0                 989 fog381
 0                 992 fog376
 0                 994 fog378
 0                 975 fog371
 0                 995 fog379
 0                 998 fog340
 0                 997 fog362
 0                 996 fog364
 0                 988 fog384
 0                 987 fog383
 0                 986 fog363
 0                 985 fog375
 0                 978 fog370
 0                 977 fog369
 0                 976 fog372
 0                 979 fog368
 0                 980 fog374
 0                 981 fog365
 0                 984 fog373
 0                 983 fog367
 0                 982 fog366
 0                 948 fog313
 0                 946 fog328
 0                 894 fcu144_3
 0                 912 faca38_1
 0                 910 fvca14_4
 0                 909 fcu72_5
 0                 908 fvca14_1
 0                 911 fvca14_5
 0                 913 faca38_4
 0                 919 fcu84_5
 0                 914 fvca14_2
 0                 917 fcu129_4
 0                 916 fcu84_3
 0                 915 fcu129_5
 0                 907 faca38_5
 0                 906 fcu84_2
 0                 905 fcu144_5
 0                 904 faca19_5
 0                 897 fcu74_2
 0                 896 fcu74_4
 0                 895 fcu144_4
 0                 898 fcu84_1
 0                 899 fcu74_1
 0                 900 faca19_1
 0                 903 faca19_4
 0                 902 faca19_3
 0                 901 faca19_2
 0                 918 fcu84_4
 0                 920 fcu129_1
 0                 945 fog327
 0                 939 fog333
 0                 937 fog324
 0                 936 fog323
 0                 935 fog316
 0                 938 fog325
 0                 940 fog336
 0                 921 fcu129_2
 0                 941 fog331
 0                 944 fog326
 0                 943 fog330
 0                 942 fog332
 0                 934 fog315
 0                 933 fog314
 0                 932 fog317
 0                 931 fog318
 0                 924 fcu140_4
 0                 923 fcu119_1
 0                 922 fcu129_3
 0                 785 faca5_3
 0                 926 fcu72_3
 0                 927 fog320
 0                 930 fog319
 0                 929 fog322
 0                 928 fog321
 0                 786 faca5_4
 0                 751 fcu1_2
 0                 784 faca5_2
 0                 642 fvn17_2
 0                 640 fcu31_4
 0                 639 fcu31_3
 0                 638 fcu31_1
 0                 641 fcu31_5
 0                 643 fvn17_3
 0                 649 faca23_5
 0                 644 fcu31_2
 0                 647 fcu71_4
 0                 646 fvn17_5
 0                 645 fcu71_5
 0                 637 fcu78_5
 0                 636 fvca14_3
 0                 635 fcu142_5
 0                 634 fcu28_2
 0                 627 fcu46_5
 0                 626 fcu28_5
 0                 624 fcu134_2
 0                 628 fcu134_3
 0                 629 fcu134_4
 0                 630 fcu134_5
 0                 633 fcu28_3
 0                 632 fcu28_4
 0                 631 fcu28_1
 0                 648 faca23_4
 0                 650 fcu71_1
 0                 620 fcu142_3
 0                 669 fvl5_3
 0                 667 fvn22_4
 0                 666 fvn22_3
 0                 665 fvl5_5
 0                 668 fvn22_5
 0                 670 fvl5_4
 0                 651 fcu71_2
 0                 671 faca23_3
 0                 674 fcu5_2
 0                 673 fcu97_1
 0                 672 faca23_1
 0                 664 fvn22_2
 0                 663 fcu56_2
 0                 662 fcu56_4
 0                 661 fcu44_4
 0                 654 fvn22_1
 0                 653 fvn17_4
 0                 652 fcu71_3
 0                 655 faca23_2
 0                 656 fcu56_3
 0                 657 fcu56_5
 0                 660 fcu44_3
 0                 659 fcu44_2
 0                 658 fcu44_1
 0                 622 fvn28_2
 0                 619 fvn36_4
 0                 676 fcu5_5
 0                 586 fcu104_3
 0                 585 fcu104_2
 0                 584 fcu78_4
 0                 583 fvn28_3
 0                 418 fvcu4_2+1
 0                 587 fcu46_1
 0                 594 fcu119_4
 0                 588 fcu104_5
 0                 592 fcu46_3
 0                 590 fvn33_1
 0                 589 fcu104_4
 0                 582 fcu111_4
 0                 580 fcu111_5
 0                 579 fvn28_4
 0                 578 fcu104_1
 0                 555 fcu132_1
 0                 488 fcu86_4
 0                 489 fcu86_5
 0                 563 fal2_2
 0                 564 fal2_3
 0                 565 fal2_4
 0                 577 fvn36_2
 0                 431 faca44_2+2
 0                 566 fal2_5
 0                 593 fcu119_3
 0                 595 fcu119_2
 0                 618 fvn36_3
 0                 613 fvn24_5
 0                 611 fcu142_2
 0                 610 fvn5_4
 0                 609 fvn5_2
 0                 612 fcu142_4
 0                 614 fvn24_4
 0                 596 fcu111_1
 0                 387 fvca8_2+0
 0                 617 fvn28_1
 0                 616 fvn36_5
 0                 615 fvn24_3
 0                 394 fvca8_1+0
 0                 608 fvn5_3
 0                 607 fvn33_5
 0                 606 fcu46_4
 0                 599 fvn33_3
 0                 598 fcu78_3
 0                 597 fvn33_4
 0                 600 fvn33_2
 0                 601 fcu78_2
 0                 602 fcu119_5
 0                 605 fcu46_2
 0                 604 fcu78_1
 0                 603 fvn28_5
 0                 675 fcu5_4
 0                 677 fcu87_1
 0                 783 faca5_1
 0                 749 fvca12_5
 0                 747 fvca3_4
 0                 746 fvca3_2
 0                 745 fcu97_3
 0                 748 fvca3_5
 0                 750 fcu1_1
 0                 757 fcu97_5
 0                 752 fvca3_3
 0                 755 fcu18_4
 0                 754 fcu1_4
 0                 753 fcu18_5
 0                 744 fvn32_2
 0                 743 fvn32_4
 0                 742 fvl4_1
 0                 741 fvl3_1
 0                 734 fvj5_3
 0                 733 fvn15_5
 0                 732 fvn15_4
 0                 735 fvj5_1
 0                 736 fvca20
 0                 737 fvl4_2
 0                 740 fvn29
 0                 739 fvn10
 0                 738 fvca19
 0                 756 fcu97_4
 0                 758 fcu18_1
 0                 730 fvj5_5
 0                 777 fvn4_5
 0                 775 fvn4_3
 0                 774 fvn4_2
 0                 773 fvn9_2
 0                 776 fvn4_4
 0                 778 fvn9_1
 0                 759 fcu18_2
 0                 779 fvca2_4
 0                 782 faca36_4
 0                 781 fcu118_3
 0                 780 fvca2_2
 0                 772 fvn4_1
 0                 771 fvn9_3
 0                 770 fvn9_5
 0                 769 faca21_5
 0                 762 fcu1_5
 0                 761 fcu1_3
 0                 760 fcu18_3
 0                 763 fvn32_1
 0                 764 fvn9_4
 0                 765 faca21_1
 0                 768 faca21_4
 0                 767 faca21_3
 0                 766 faca21_2
 0                 731 fvn15_3
 0                 729 fvj5_4
 0                 678 fcu87_2
 0                 696 faca4_1
 0                 694 faca39_3
 0                 693 faca39_2
 0                 692 fcu98_5
 0                 695 faca39_4
 0                 697 faca4_2
 0                 703 fcu149_4
 0                 698 faca39_1
 0                 701 fcu98_3
 0                 700 fcu149_2
 0                 699 fcu98_4
 0                 691 faca4_3
 0                 690 fcu149_1
 0                 689 fcu87_4
 0                 688 fvl6_4
 0                 681 fcu5_1
 0                 680 fcu5_3
 0                 679 fcu87_3
 0                 682 fcu87_5
 0                 683 fvl6_5
 0                 684 fvca2_5
 0                 687 fvl6_3
 0                 686 fvl6_2
 0                 685 fvl6_1
 0                 702 fcu149_3
 0                 704 fcu149_5
 0                 728 fvj5_2
 0                 722 fvn35_3
 0                 720 fvn35_1
 0                 719 fvn23_2
 0                 718 fvn18_4
 0                 721 fvn35_2
 0                 723 fvn35_4
 0                 705 fcu98_1
 0                 724 fvn23_1
 0                 727 fvn32_3
 0                 726 fvn21
 0                 725 fvn18_3
 0                 717 fvn23_3
 0                 716 fvn3_1
 0                 715 fvn18_2
 0                 714 fvn18_1
 0                 708 fcu97_2
 0                 707 fcu44_5
 0                 706 fcu98_2
 0                 709 fvca2_3
 0                 291 fog188
 0                 710 fvn23_4
 0                 713 fvn3_4
 0                 712 fvn3_3
 0                 711 fvn3_2
 0                1000 fog348

Selected attributes: 1,2,3,4,5,6,8,7,9,11,10,12,14,13,15,16,17,18,19,20,24,21,23,25,26,27,22,28,32,31,33,36,40,29,30,35,34,38,41,39,42,43,45,46,49,47,50,52,51,37,54,53,55,56,57,58,59,60,61,44,48,62,63,64,65,66,68,67,69,70,71,72,74,73,78,75,76,77,79,80,81,82,83,85,84,87,88,89,86,90,91,93,94,92,95,97,96,98,99,100,101,104,102,103,108,105,107,106,109,110,111,112,113,115,114,116,117,118,119,120,121,122,123,124,125,126,127,128,129,130,132,131,133,135,137,134,136,141,139,138,140,142,143,144,145,146,147,148,149,150,152,151,153,156,157,155,159,158,154,160,163,164,162,165,161,166,167,168,177,169,170,173,172,171,174,175,176,178,193,179,195,180,181,182,191,186,189,190,184,188,187,185,183,192,194,196,206,217,197,198,199,200,204,205,202,203,201,207,208,209,210,212,213,214,215,211,216,218,219,220,221,222,223,224,225,229,227,228,226,230,232,234,231,233,243,236,235,242,237,239,241,253,240,238,248,245,246,247,250,251,252,244,249,255,254,256,257,259,258,260,262,261,263,264,271,265,266,267,268,269,270,272,273,274,275,276,277,278,279,280,281,282,283,284,285,286,287,299,288,289,290,292,293,294,295,297,296,298,311,343,300,302,301,326,327,312,329,303,304,322,315,316,307,306,305,309,308,334,310,314,392,341,342,313,323,317,318,319,320,321,325,324,331,328,330,338,332,333,336,335,337,340,339,385,345,372,373,370,371,365,374,368,367,369,377,375,382,384,383,381,378,380,379,366,376,364,352,353,363,351,350,349,347,346,354,348,355,360,361,356,359,362,358,357,386,389,344,388,391,393,395,396,400,399,397,398,405,402,404,403,401,390,406,407,408,413,410,409,411,412,414,422,417,416,415,419,421,420,424,423,425,426,428,429,430,427,432,433,434,456,436,435,466,437,439,440,438,442,444,443,441,446,447,448,449,445,451,450,452,453,454,455,464,457,460,458,459,461,462,465,463,467,469,470,468,471,472,473,474,475,476,477,478,479,480,481,482,483,484,486,485,487,490,493,492,491,494,495,496,497,498,499,501,502,503,533,504,505,506,507,508,500,509,510,512,511,513,514,515,516,517,549,537,518,519,520,521,522,524,523,525,526,527,528,530,529,531,532,534,536,535,538,539,832,543,542,540,541,544,545,546,548,547,550,551,553,552,625,554,621,556,557,558,559,827,561,560,591,581,562,623,568,567,569,570,572,573,571,575,574,576,853,852,840,855,851,854,858,856,859,850,857,887,888,849,843,841,889,890,842,844,848,845,847,860,846,886,864,861,874,878,877,876,884,879,880,883,882,881,875,873,862,872,866,865,863,867,868,885,871,870,869,999,809,839,804,802,801,800,803,805,838,806,892,808,807,799,798,797,796,789,788,787,790,791,792,795,794,793,810,811,812,825,830,829,828,831,833,834,837,836,835,826,824,813,823,816,815,814,817,818,819,822,821,820,891,925,893,966,964,963,962,965,967,973,968,971,970,969,961,960,959,958,951,950,949,952,953,954,957,956,955,972,974,947,993,991,990,989,992,994,975,995,998,997,996,988,987,986,985,978,977,976,979,980,981,984,983,982,948,946,894,912,910,909,908,911,913,919,914,917,916,915,907,906,905,904,897,896,895,898,899,900,903,902,901,918,920,945,939,937,936,935,938,940,921,941,944,943,942,934,933,932,931,924,923,922,785,926,927,930,929,928,786,751,784,642,640,639,638,641,643,649,644,647,646,645,637,636,635,634,627,626,624,628,629,630,633,632,631,648,650,620,669,667,666,665,668,670,651,671,674,673,672,664,663,662,661,654,653,652,655,656,657,660,659,658,622,619,676,586,585,584,583,418,587,594,588,592,590,589,582,580,579,578,555,488,489,563,564,565,577,431,566,593,595,618,613,611,610,609,612,614,596,387,617,616,615,394,608,607,606,599,598,597,600,601,602,605,604,603,675,677,783,749,747,746,745,748,750,757,752,755,754,753,744,743,742,741,734,733,732,735,736,737,740,739,738,756,758,730,777,775,774,773,776,778,759,779,782,781,780,772,771,770,769,762,761,760,763,764,765,768,767,766,731,729,678,696,694,693,692,695,697,703,698,701,700,699,691,690,689,688,681,680,679,682,683,684,687,686,685,702,704,728,722,720,719,718,721,723,705,724,727,726,725,717,716,715,714,708,707,706,709,291,710,713,712,711,1000 : 1000



==> docs/static_features_info_gain <==
=== Run information ===

Evaluator:    weka.attributeSelection.InfoGainAttributeEval 
Search:       weka.attributeSelection.Ranker -T -1.7976931348623157E308 -N -1
Relation:     keyword_features-weka.filters.unsupervised.attribute.PartitionedMultiFilter-Fweka.filters.supervised.attribute.AttributeSelection -E "weka.attributeSelection.InfoGainAttributeEval " -S "weka.attributeSelection.Ranker -T -1.7976931348623157E308 -N 1000"-R3-last-weka.filters.unsupervised.attribute.RenameAttribute-find^(filtered-0-|unfiltered-)(/\w+)+$-replace$2-Rfirst-last-weka.filters.unsupervised.attribute.RenameAttribute-find^(filtered-0-|unfiltered-)(\w+)+$-replace$2-Rfirst-last-weka.filters.unsupervised.attribute.Reorder-R1002,1003,first-1001-weka.filters.unsupervised.attribute.Remove-R1-2
Instances:    143526
Attributes:   1001
              [list of attributes omitted]
Evaluation mode:    evaluate on all training data



=== Attribute Selection on all input data ===

Search Method:
	Attribute ranking.

Attribute Evaluator (supervised, Class (nominal): 1001 class):
	Information Gain Ranking Filter

    f9458,Literal:alphabetic (detail https://developer.mozilla.org/en-US/docs/Web/SVG/Attribute/alphabetic)
    f45965,AssignmentExpression:alphabetic
    f61,Literal:canvas
    f14509,Literal:ActiveXObject
    f34491,MemberExpression:getSupportedExtensions
    f9842,MemberExpression:toDataURL
    f8020,MemberExpression:fillText
    f4601,Identifier:getSupportedExtensions
    
Ranked attributes:
 0.017682       3 f9458
 0.017078       4 f45965
 0.015486       1 f61
 0.015142       2 f14509
 0.014871       6 f34491
 0.014824       7 f9842
 0.014824       9 f8020
 0.014752       8 f4601
 0.014646      10 f7027
 0.014606      11 f43315
 0.014325      12 f7242
 0.014325      13 f8797
 0.014093      14 f36402
 0.013772      15 f20428
 0.013718      17 f16277
 0.013505      20 f22947
 0.013466       5 f38260
 0.013438      16 f3856
 0.013419      21 f25700
 0.013382      19 f22347
 0.013341      18 f42465
 0.013241      23 f29032
 0.013208      22 f17595
 0.013017      24 f13251
 0.012838      25 f41232
 0.012814      27 f12482
 0.012737      28 f26121
 0.012478      34 f18110
 0.012278      35 f26070
 0.012258      26 f32985
 0.012161      32 f11644
 0.012091      39 f13183
 0.012054      38 f46133
 0.012054      31 f16290
 0.011954      41 f16408
 0.011888      42 f7259
 0.011888      43 f26097
 0.01184       45 f38301
 0.011837      36 f33679
 0.011804      48 f22177
 0.011768      52 f39889
 0.011703      37 f27584
 0.011679      53 f23660
 0.011652      84 f26659
 0.011642      54 f227
 0.011623      46 f14422
 0.01162       62 f23254
 0.011612      64 f27366
 0.011605      59 f46954
 0.011604      55 f11845
 0.011603      60 f20872
 0.011599      61 f3102
 0.011591      58 f40460
 0.01159       56 f8612
 0.011574      57 f19124
 0.011573      50 f12359
 0.011553      70 f41476
 0.011541      89 f40357
 0.01154       71 f37114
 0.011535      66 f15962
 0.011526      67 f8545
 0.011522      69 f37825
 0.011522      83 f38876
 0.011521      75 f5036
 0.011515      65 f29568
 0.011505      63 f11367
 0.011504      72 f45834
 0.011499      68 f34483
 0.011498      74 f32539
 0.01147       82 f33525
 0.011462      73 f8478
 0.011457      78 f22922
 0.011456      76 f28459
 0.011455      79 f5361
 0.011425      80 f24089
 0.011423      85 f26261
 0.011423      86 f10234
 0.011421      81 f14690
 0.011415      44 f3130
 0.011367      87 f43044
 0.011359      77 f42429
 0.011352      51 f2241
 0.011326      88 f28171
 0.011255      90 f43500
 0.011243      49 f4375
 0.011202      92 f3904
 0.011175      94 f2225
 0.011124      96 f32153
 0.011122      95 f29491
 0.010964      98 f7973
 0.010837      97 f39483
 0.010546     100 f6859
 0.010192     107 f28029
 0.009822     103 f15606
 0.009716     115 f35333
 0.00969      111 f18142
 0.009662     116 f29068
 0.00951      118 f44676
 0.009448     117 f3683
 0.009417     119 f9670
 0.009392      29 f30387
 0.009375     120 f26356
 0.009336     125 f16112
 0.00928      128 f8963
 0.009228     121 f17050
 0.009191     122 f42256
 0.009185     140 f21918
 0.009169      33 f36412
 0.009139     124 f6679
 0.009044     145 f14984
 0.008898     127 f13609
 0.008861     141 f29654
 0.008819      40 f11225
 0.008814     139 f44837
 0.008753     130 f23241
 0.008728     132 f30111
 0.008604     135 f40816
 0.008562     142 f43369
 0.008509     114 f27682
 0.008271      30 f30610
 0.008264     154 f18751
 0.008224      91 f40022
 0.008148     162 f44063
 0.007814     169 f7279
 0.007789     168 f17365
 0.007742      99 f15665
 0.007653      47 f14534
 0.007588     104 f11022
 0.007584     175 f1967
 0.00752      192 f20744
 0.007482     176 f21611
 0.007452     109 f35552
 0.007449     158 f14587
 0.00743       93 f33459
 0.007394     156 f9867
 0.007386     184 f2500
 0.00733      182 f26749
 0.007284     183 f8818
 0.007276     185 f26081
 0.007272     166 f36479
 0.007207     165 f632
 0.00717      199 f11443
 0.006966     200 f38352
 0.006964     207 f13816
 0.006901     195 f35054
 0.006828     102 f4570
 0.006742     208 f13216
 0.006681     101 f37885
 0.006655     106 f13016
 0.006583     113 f7831
 0.006553     105 f8864
 0.006519     134 f45826
 0.006289     225 f10678
 0.006241     112 f43904
 0.006204     110 f39836
 0.006189     108 f5227
 0.006167     219 f11851
 0.005916     123 f33571
 0.005774     236 f40974
 0.005714     126 f8493
 0.005689     153 f19990
 0.00567      129 f24320
 0.005635     238 f41466
 0.005609     133 f31327
 0.005454     245 f22594
 0.005405     136 f46778
 0.005391     131 f29463
 0.005384     137 f46107
 0.00537      209 f3722
 0.005348     138 f28856
 0.005258     187 f34843
 0.005249     147 f6091
 0.005233     157 f4581
 0.005216     144 f21673
 0.005209     150 f24836
 0.005208     253 f7137
 0.005197     143 f33844
 0.005194     247 f46637
 0.005188     160 f14302
 0.005122     155 f45491
 0.005079     148 f29286
 0.005073     151 f40721
 0.005038     167 f28784
 0.005029     254 f20312
 0.005029     235 f46127
 0.005002     146 f24722
 0.004947     149 f26495
 0.004936     159 f13630
 0.00489      239 f13054
 0.004842     260 f47622
 0.004799     251 f16802
 0.004783     171 f34122
 0.004779     170 f22215
 0.004751     161 f1143
 0.004737     152 f38327
 0.004732     164 f46587
 0.00466      263 f28158
 0.004649     163 f40208
 0.004635     177 f18001
 0.004622     178 f10175
 0.004615     202 f30891
 0.004588     268 f33149
 0.004528     188 f47381
 0.004521     172 f43118
 0.004481     179 f16570
 0.004467     173 f9798
 0.004439     180 f17673
 0.004359     201 f21531
 0.004353     174 f29956
 0.004341     271 f3792
 0.004313     270 f37350
 0.004305     266 f13874
 0.004295     186 f23652
 0.004266     181 f27781
 0.004258     193 f570
 0.004163     190 f30071
 0.004151     276 f33727
 0.004084     189 f14583
 0.004079     214 f9089
 0.004072     196 f4463
 0.004031     287 f4064
 0.004015     191 f37428
 0.004002     274 f777
 0.003999     222 f24345
 0.003994     216 f3192
 0.00398      211 f14510
 0.003958     204 f36775
 0.003941     194 f14156
 0.00392      197 f20979
 0.003885     210 f10184
 0.003875     206 f1651
 0.003866     291 f20022
 0.003854     231 f36526
 0.003817     203 f37183
 0.003816     198 f16869
 0.003812     205 f965
 0.003728     217 f34330
 0.003689     223 f833
 0.003679     218 f2343
 0.003673     213 f6994
 0.00366      215 f18091
 0.003649     212 f25916
 0.003619     230 f6922
 0.003614     221 f45352
 0.0036       314 f34152
 0.003587     224 f45347
 0.003523     220 f34864
 0.003514     233 f46191
 0.003496     226 f37185
 0.003431     310 f28217
 0.003398     227 f34949
 0.003378     324 f17308
 0.003369     232 f1314
 0.003353     241 f8144
 0.00335      234 f17196
 0.003341     229 f27779
 0.003334     228 f4408
 0.00332      312 f20009
 0.003312     330 f16827
 0.003307     246 f23752
 0.0033       302 f23024
 0.003276     303 f39348
 0.003241     240 f23273
 0.003201     256 f7117
 0.003198     237 f2159
 0.003173     320 f34950
 0.00316      248 f45261
 0.003154     332 f14464
 0.00313      356 f26442
 0.003125     318 f9535
 0.003088     244 f5994
 0.003086     360 f43582
 0.003075     243 f37518
 0.003042     257 f31900
 0.003001     327 f36793
 0.002911     265 f40096
 0.002898     242 f36711
 0.002863     250 f47500
 0.002858     272 f35491
 0.002846     252 f4206
 0.002835     281 f24034
 0.002834     249 f8786
 0.002833     361 f40583
 0.002826     279 f4484
 0.002806     267 f29120
 0.002782     282 f4840
 0.002764     283 f14307
 0.002756     264 f23877
 0.002753     258 f14145
 0.002751     313 f1338
 0.00274      364 f44113
 0.002732     307 f6650
 0.00273      298 f32352
 0.002725     355 f20203
 0.00272      255 f9297
 0.002714     284 f20700
 0.00271      317 f40479
 0.002708     285 f44653
 0.002708     277 f29533
 0.002678     269 f22024
 0.002673     300 f12038
 0.002661     389 f40159
 0.002652     290 f5489
 0.002645     259 f21166
 0.002644     288 f20077
 0.002638     262 f39427
 0.002622     292 f36883
 0.002621     308 f17003
 0.002578     261 f10441
 0.00257      395 f12227
 0.002569     325 f842
 0.002565     370 f31646
 0.002564     396 f28480
 0.002513     297 f37240
 0.00249      333 f40573
 0.002487     304 f37491
 0.002449     371 f25044
 0.002448     273 f12654
 0.002443     400 f40343
 0.002402     378 f2580
 0.002382     278 f35451
 0.00238      336 f12339
 0.002376     305 f2240
 0.002373     385 f10443
 0.002361     349 f41094
 0.00236      280 f17456
 0.002345     294 f16628
 0.002334     341 f27579
 0.002329     316 f23193
 0.002327     315 f10475
 0.002325     275 f34207
 0.002303     391 f43456
 0.002277     365 f21640
 0.002277     322 f13370
 0.002253     328 f7837
 0.002221     286 f42370
 0.002219     326 f34274
 0.002208     342 f22968
 0.002165     289 f5432
 0.002165     311 f23758
 0.002134     335 f44768
 0.00213      363 f25398
 0.002097     295 f40559
 0.002081     353 f6112
 0.002079     346 f6833
 0.002052     343 f26740
 0.002051     296 f38152
 0.002042     309 f24979
 0.002034     369 f14740
 0.002009     319 f10380
 0.002004     430 f27768
 0.002002     403 f45284
 0.001994     323 f15186
 0.001992     339 f24891
 0.001971     424 f9347
 0.001959     381 f5344
 0.001942     301 f46612
 0.001934     340 f7168
 0.001907     293 f15602
 0.0019       299 f36850
 0.001867     387 f40630
 0.001863     447 f38807
 0.001855     429 f13925
 0.001832     468 f22812
 0.001815     475 f37303
 0.001794     331 f2025
 0.001773     474 f9005
 0.00176      344 f31306
 0.001754     489 f19383
 0.001736     477 f19016
 0.001724     306 f4696
 0.001697     337 f7811
 0.001689     520 f8896
 0.001677     469 f39136
 0.00167      338 f37809
 0.001654     358 f43374
 0.001627     345 f19654
 0.001623     376 f10140
 0.001615     483 f17335
 0.001613     321 f9848
 0.001603     388 f41297
 0.001602     380 f39066
 0.001601     350 f32487
 0.001589     351 f20590
 0.00156      348 f40762
 0.001552     347 f23505
 0.00154      384 f33608
 0.001522     383 f5412
 0.001495     374 f18064
 0.001489     402 f18033
 0.00147      419 f37477
 0.001466     516 f16594
 0.001456     417 f34446
 0.001454     406 f26522
 0.001453     368 f39391
 0.00143      530 f31796
 0.001421     366 f43223
 0.001413     571 f4252
 0.001407     422 f8416
 0.001402     394 f43189
 0.001385     545 f10797
 0.001377     382 f45373
 0.001366     379 f33213
 0.001365     440 f712
 0.001349     690 f10855
 0.001335     329 f4777
 0.001326     390 f31583
 0.001323     362 f12779
 0.001313     593 f32591
 0.001311     392 f33521
 0.00131      525 f31768
 0.001291     465 f3157
 0.001286     412 f31294
 0.001277     555 f27870
 0.001272     334 f45117
 0.001271     413 f4084
 0.001265     357 f41567
 0.001252     359 f27437
 0.001252     375 f18275
 0.001248     367 f30309
 0.001223     615 f45685
 0.001221     377 f38518
 0.001216     404 f21832
 0.001187     529 f36738
 0.00117      749 f43665
 0.001157     397 f31753
 0.001145     398 f42345
 0.001145     498 f45939
 0.001128     554 f45294
 0.001127     386 f17059
 0.001126     619 f33692
 0.001126     441 f22166
 0.001111     601 f35102
 0.001111     354 f18397
 0.001106     742 f38477
 0.001104     352 f2979
 0.001095     446 f26569
 0.001095     612 f27562
 0.00109      467 f17362
 0.001087     372 f46072
 0.001087     452 f31026
 0.001087     460 f32163
 0.001084     393 f6992
 0.001079     445 f11312
 0.001079     471 f31079
 0.001077     457 f17183
 0.001075     656 f38276
 0.001064     408 f44773
 0.001058     827 f5795
 0.001056     373 f38057
 0.001048     459 f24808
 0.001047     470 f42840
 0.001045     454 f26146
 0.001036     420 f11772
 0.00103      401 f1287
 0.001027     462 f26537
 0.001011     755 f9531
 0.000999     500 f12624
 0.000997     482 f44011
 0.00099      415 f14940
 0.000986     553 f4024
 0.000981     428 f20049
 0.000981     598 f29095
 0.000967     487 f28256
 0.000948     563 f30519
 0.000933     509 f14894
 0.000931     521 f15161
 0.000927     565 f14855
 0.000925     607 f23301
 0.000909     405 f34210
 0.000895     960 f19019
 0.000888     506 f42866
 0.000884     624 f32970
 0.000879     561 f35142
 0.000868     399 f41155
 0.000867     476 f18328
 0.000845     464 f39761
 0.000841     432 f29253
 0.000829     479 f6427
 0.000825     414 f45527
 0.000822     536 f9920
 0.000821     463 f33610
 0.000818     411 f24674
 0.000814     484 f47345
 0.000813     834 f20885
 0.000807     416 f41290
 0.000805     410 f13845
 0.000802     427 f15204
 0.0008       421 f44258
 0.0008       407 f11146
 0.000796     425 f12091
 0.000793     585 f39160
 0.000792     663 f29790
 0.000791     433 f26661
 0.000787     857 f26538
 0.00078      431 f9537
 0.000778     673 f23040
 0.000778     443 f33902
 0.000777     461 f6012
 0.000776     418 f44317
 0.000766     437 f1418
 0.000762     409 f22343
 0.000752     480 f18699
 0.000751     730 f26711
 0.000748     436 f556
 0.000744     448 f44621
 0.000742     794 f40310
 0.000736     717 f13525
 0.000731     435 f34793
 0.000729     513 f39685
 0.000727     423 f44255
 0.000726     466 f47426
 0.000724     494 f12513
 0.000723     752 f11278
 0.000722     458 f38325
 0.00072      646 f46362
 0.00072      645 f34862
 0.000719     634 f20156
 0.000718     740 f46833
 0.000715     586 f5347
 0.000712     835 f42451
 0.000706     528 f7642
 0.000703     478 f6893
 0.000703     438 f6478
 0.000702     456 f21738
 0.0007       434 f4250
 0.000699     451 f37922
 0.000689     450 f3484
 0.000687     975 f12102
 0.000683     594 f29276
 0.000681     584 f11558
 0.000677     444 f13479
 0.000676     973 f43087
 0.000675     449 f31971
 0.000668     790 f37735
 0.000668     517 f47624
 0.000668     580 f26701
 0.000661     439 f7217
 0.00066      473 f18837
 0.000656     426 f14114
 0.000652     772 f35556
 0.00065      628 f1567
 0.000646     562 f1030
 0.000641     620 f36007
 0.000636     640 f33215
 0.000635     626 f27993
 0.000633     892 f30590
 0.000633     650 f14988
 0.000633     486 f25539
 0.00063      442 f11243
 0.000627     534 f14905
 0.000627     683 f24047
 0.000627     682 f1592
 0.000627     621 f39229
 0.000626     710 f9692
 0.000626     685 f5779
 0.000625     660 f39635
 0.000625     453 f22391
 0.000625     662 f29557
 0.000625     687 f42210
 0.000624     455 f39118
 0.000624     499 f46617
 0.000623     568 f43327
 0.000623     671 f4435
 0.000623     505 f14626
 0.000622     495 f42009
 0.000622     681 f41488
 0.000619     485 f26927
 0.000618     688 f32830
 0.000616     694 f18775
 0.000615     670 f12742
 0.000614     504 f12080
 0.000614     501 f16745
 0.000614     492 f35443
 0.000612     691 f43064
 0.000611     488 f11761
 0.000611     692 f34016
 0.000611     712 f14791
 0.000611     623 f21476
 0.00061      543 f21985
 0.000608     546 f10752
 0.000608     544 f9300
 0.000607     493 f10896
 0.000602     978 f14603
 0.0006       693 f32390
 0.000599     507 f12476
 0.000598     508 f36332
 0.000598     695 f8650
 0.000598     804 f18878
 0.000598     539 f14089
 0.000598     524 f38291
 0.000597     514 f44510
 0.000597     743 f25338
 0.000596     502 f29160
 0.000593     497 f24446
 0.000592     527 f30447
 0.000587     496 f5324
 0.000586     674 f42393
 0.000583     732 f11629
 0.000581     518 f13748
 0.000581     519 f154
 0.000579     511 f2634
 0.000579     512 f37379
 0.000578     515 f19152
 0.000573     541 f33229
 0.00057      707 f9677
 0.000568     731 f28470
 0.000568     540 f32825
 0.000566     741 f9000
 0.000565     532 f24897
 0.000563     643 f17263
 0.000562     747 f35204
 0.000561     667 f10553
 0.000559     675 f25104
 0.000557     705 f37433
 0.000557     526 f8768
 0.000557     728 f5605
 0.000556     766 f10989
 0.000554     679 f13351
 0.000554     491 f9546
 0.000552     481 f28177
 0.000551     988 f24558
 0.000551     644 f32453
 0.000551     706 f44889
 0.00055      997 f13347
 0.000547     696 f21742
 0.000547     727 f4539
 0.000547     652 f5147
 0.000542     625 f47383
 0.000542     699 f16769
 0.000541     797 f37017
 0.00054      552 f40347
 0.000522     893 f25685
 0.000519     799 f12627
 0.000517     510 f45340
 0.000516     574 f47575
 0.000512     744 f14578
 0.000508     590 f7854
 0.000508     573 f20843
 0.000508     591 f25049
 0.000506     769 f40302
 0.000505     572 f8799
 0.000503     665 f40779
 0.000502     533 f9884
 0.0005       550 f12126
 0.000498     664 f20240
 0.000496     559 f5910
 0.000496     853 f1922
 0.000494     855 f25859
 0.000492     916 f38275
 0.00049      567 f9926
 0.00049      522 f31791
 0.00049      654 f34620
 0.000489     589 f316
 0.000489     631 f35334
 0.000488     709 f28427
 0.000488     716 f34754
 0.000484     639 f10291
 0.000483     503 f31815
 0.000483     564 f22175
 0.000482     819 f21132
 0.00048      547 f47264
 0.000478     581 f37525
 0.000477     711 f35185
 0.000477     537 f34659
 0.000477     669 f20223
 0.000475     596 f6387
 0.000475     829 f26307
 0.000475     551 f36114
 0.000474     622 f33992
 0.000474     759 f41672
 0.000471     592 f4975
 0.000471     538 f42077
 0.000469     560 f47255
 0.000469     651 f36756
 0.000469     704 f36107
 0.000468     523 f3370
 0.000465     490 f25465
 0.000465     945 f1159
 0.000464     764 f14423
 0.000464     816 f22096
 0.000464     556 f17178
 0.000464     641 f22417
 0.000463     472 f41874
 0.000463     558 f16151
 0.000462     800 f1231
 0.000458     576 f37082
 0.000458     531 f9197
 0.000457     735 f18919
 0.000457     871 f14013
 0.000454     856 f24031
 0.000454     784 f12415
 0.000454     795 f41243
 0.000453     566 f42390
 0.00045      822 f32651
 0.000449     600 f29239
 0.000448     783 f15100
 0.000447     770 f5873
 0.000446     761 f11638
 0.000444     721 f10641
 0.000443     535 f36952
 0.000443     739 f3926
 0.000443     610 f26972
 0.000443     583 f14138
 0.000442     569 f11561
 0.000441     653 f38960
 0.000441     548 f41920
 0.000438     899 f18249
 0.000438     817 f32463
 0.000438     575 f20835
 0.000434     773 f46157
 0.000431     604 f44801
 0.00043      808 f10893
 0.000427     883 f30378
 0.000427     861 f10386
 0.000424     549 f16814
 0.000424     722 f42291
 0.000421     570 f37074
 0.000421     577 f16872
 0.00042      648 f9813
 0.00042      647 f20090
 0.000418     737 f36946
 0.000417     748 f33685
 0.000417     617 f23512
 0.000416     659 f42340
 0.000414     542 f7228
 0.000413     760 f35358
 0.000413     895 f37059
 0.000413     595 f15514
 0.000412     627 f32577
 0.000412     587 f15763
 0.000411     858 f34833
 0.000409     629 f2679
 0.000406     698 f34895
 0.000405     859 f41790
 0.000403     636 f23557
 0.000401     792 f20581
 0.000401     613 f6396
 0.0004       891 f25947
 0.000399     676 f26750
 0.000399     677 f44580
 0.000399     811 f17062
 0.000398     798 f39477
 0.000397     757 f21851
 0.000397     609 f771
 0.000396     702 f31765
 0.000392     841 f280
 0.00039      904 f23167
 0.000387     678 f8301
 0.000386     802 f15823
 0.000386     700 f14220
 0.000385     703 f32673
 0.000385     599 f10637
 0.000385     597 f41921
 0.000385     655 f42220
 0.000384     845 f26679
 0.000381     738 f3736
 0.00038      680 f18485
 0.00038      668 f11105
 0.000378     726 f9582
 0.000374     734 f14774
 0.000372     557 f13293
 0.000371     860 f9758
 0.000369     684 f47320
 0.000368     579 f17949
 0.000368     762 f38920
 0.000368     932 f7107
 0.000367     907 f9327
 0.000363     578 f8112
 0.000362     642 f26351
 0.000362     729 f32578
 0.000362     672 f9819
 0.000358    1000 f27720
 0.000358     718 f26502
 0.000357     927 f7373
 0.000356     863 f7007
 0.000356     864 f1571
 0.000353     894 f33377
 0.000351     697 f7937
 0.000351     611 f27837
 0.00035      608 f37778
 0.000349     701 f47265
 0.000349     632 f4030
 0.000347     714 f34359
 0.000347     666 f8439
 0.000346     602 f11347
 0.000345     633 f2604
 0.000345     831 f22105
 0.000345     939 f32987
 0.000344     713 f21898
 0.000344     758 f41604
 0.000344     614 f1667
 0.000343     815 f14870
 0.000343     881 f36413
 0.000343     814 f13082
 0.000342     897 f12759
 0.000342     603 f37507
 0.000342     605 f37694
 0.000341     789 f24434
 0.000339     999 f29630
 0.000338     896 f13389
 0.000336     913 f22338
 0.000334     649 f38024
 0.000334     952 f37310
 0.000333     588 f7906
 0.000333     791 f37793
 0.000333     724 f29085
 0.000332     990 f40327
 0.000332     689 f15821
 0.000332     637 f20324
 0.00033      638 f41975
 0.00033      879 f29484
 0.00033      949 f44292
 0.000329     911 f43594
 0.000329     793 f10717
 0.000329     616 f42133
 0.000328     635 f40667
 0.000328     887 f16312
 0.000328     745 f7740
 0.000328     657 f15759
 0.000328     846 f26712
 0.000327     750 f32510
 0.000327     582 f930
 0.000326     776 f26866
 0.000325     968 f15799
 0.000325     686 f19985
 0.000325     779 f22848
 0.000325     780 f42398
 0.000324     944 f32518
 0.000322     715 f26922
 0.000322     812 f25102
 0.000321     805 f24823
 0.00032      708 f15997
 0.00032      661 f5060
 0.00032      719 f11421
 0.00032      720 f43519
 0.000318     925 f9366
 0.000317     962 f26007
 0.000317     974 f40381
 0.000317     832 f4364
 0.000317     630 f14078
 0.000314     723 f16047
 0.000312     606 f47029
 0.000311     961 f15744
 0.000309     763 f43094
 0.000308     828 f13896
 0.000307     733 f23347
 0.000307     971 f25646
 0.000306     751 f41631
 0.000306     775 f28071
 0.000304     874 f8388
 0.000303     736 f112
 0.000302     984 f15025
 0.000302     618 f45134
 0.000302     746 f29254
 0.000301     866 f30568
 0.000301     765 f1063
 0.0003       753 f26529
 0.0003       754 f33639
 0.000299     959 f8887
 0.000299     781 f24920
 0.000298     886 f5424
 0.000297     998 f21610
 0.000296     756 f46512
 0.000294     767 f13971
 0.000293     838 f26194
 0.000293     796 f13669
 0.000293     982 f30693
 0.000293     803 f384
 0.000292     900 f34583
 0.000291     809 f46843
 0.000291     989 f29758
 0.00029      786 f35937
 0.000289     842 f35312
 0.000288     844 f10521
 0.000287     777 f35633
 0.000287     935 f40226
 0.000286     771 f20446
 0.000285     934 f23286
 0.000285     810 f24171
 0.000284     867 f1157
 0.000284     943 f44364
 0.000281     843 f41776
 0.000278     885 f6115
 0.000277     820 f44517
 0.000277     782 f26892
 0.000276     868 f14239
 0.000276     725 f29928
 0.000275     658 f26542
 0.000274     852 f18116
 0.000274     955 f3873
 0.000272     983 f26197
 0.000272     963 f1403
 0.000269     931 f24400
 0.000265     950 f5058
 0.000265     801 f45760
 0.000264     957 f32023
 0.000264     884 f25128
 0.000262     785 f29079
 0.000261     875 f6936
 0.000261     824 f18802
 0.00026      854 f24871
 0.00026      869 f9886
 0.000259     818 f33605
 0.000257     825 f47680
 0.000256     888 f27126
 0.000255     929 f32979
 0.000254     877 f29686
 0.000254     862 f38745
 0.000254     806 f38572
 0.000254     880 f19743
 0.000253     922 f6826
 0.000253     905 f10051
 0.000252     926 f14378
 0.000252     788 f9555
 0.000251     821 f36704
 0.000249     994 f1611
 0.000248     882 f38244
 0.000246     849 f42098
 0.000246     914 f21533
 0.000246     787 f33111
 0.000245     839 f32060
 0.000244     902 f1058
 0.000244     979 f43280
 0.000243     903 f31651
 0.000243     830 f41023
 0.000242     920 f264
 0.000242     947 f1840
 0.00024      876 f35487
 0.00024      878 f1152
 0.000239     995 f43899
 0.000238     833 f1828
 0.000236     996 f43476
 0.000236     919 f25907
 0.000235     872 f38277
 0.000235     807 f9756
 0.000233     970 f17479
 0.000232     924 f22595
 0.000232     940 f24124
 0.000232     928 f13120
 0.000229     836 f8005
 0.000228     778 f19161
 0.000227     915 f6918
 0.000226     930 f29106
 0.000226     981 f25204
 0.000225     890 f23081
 0.000225     865 f11279
 0.000221     917 f21802
 0.00022      937 f13513
 0.000219     954 f46820
 0.000218     938 f11159
 0.000217     768 f8883
 0.000216     933 f12521
 0.000215     993 f7177
 0.000214     901 f5947
 0.000213     840 f196
 0.000212     921 f31308
 0.000212     908 f45138
 0.00021      910 f21608
 0.000207     967 f14133
 0.000207     987 f39576
 0.000207     912 f41359
 0.000206     873 f44933
 0.000206     870 f8986
 0.000205     823 f47136
 0.000203     848 f3638
 0.000203     965 f33966
 0.000202     813 f1080
 0.0002       918 f1186
 0.0002       977 f28078
 0.000199     992 f17230
 0.000199     850 f47393
 0.000198     958 f4382
 0.000198     851 f21887
 0.000198     909 f43324
 0.000196     969 f26467
 0.000193     826 f34188
 0.000192     941 f19823
 0.000191     991 f12360
 0.000191     774 f33886
 0.000188     972 f14123
 0.000188     837 f3138
 0.000187     847 f16546
 0.000184     906 f4802
 0.000184     986 f43198
 0.000182     889 f28110
 0.000182     936 f15687
 0.000179     923 f31702
 0.000174     898 f9782
 0.000174     964 f15565
 0.000172     942 f44643
 0.000171     953 f10067
 0.000166     948 f3475
 0.000159     946 f20870
 0.000153     951 f4362
 0.000152     956 f43729
 0.000152     966 f26213
 0.000146     980 f13139
 0.000146     976 f38782
 0.000145     985 f40901

Selected attributes: 3,4,1,2,6,7,9,8,10,11,12,13,14,15,17,20,5,16,21,19,18,23,22,24,25,27,28,34,35,26,32,39,38,31,41,42,43,45,36,48,52,37,53,84,54,46,62,64,59,55,60,61,58,56,57,50,70,89,71,66,67,69,83,75,65,63,72,68,74,82,73,78,76,79,80,85,86,81,44,87,77,51,88,90,49,92,94,96,95,98,97,100,107,103,115,111,116,118,117,119,29,120,125,128,121,122,140,33,124,145,127,141,40,139,130,132,135,142,114,30,154,91,162,169,168,99,47,104,175,192,176,109,158,93,156,184,182,183,185,166,165,199,200,207,195,102,208,101,106,113,105,134,225,112,110,108,219,123,236,126,153,129,238,133,245,136,131,137,209,138,187,147,157,144,150,253,143,247,160,155,148,151,167,254,235,146,149,159,239,260,251,171,170,161,152,164,263,163,177,178,202,268,188,172,179,173,180,201,174,271,270,266,186,181,193,190,276,189,214,196,287,191,274,222,216,211,204,194,197,210,206,291,231,203,198,205,217,223,218,213,215,212,230,221,314,224,220,233,226,310,227,324,232,241,234,229,228,312,330,246,302,303,240,256,237,320,248,332,356,318,244,360,243,257,327,265,242,250,272,252,281,249,361,279,267,282,283,264,258,313,364,307,298,355,255,284,317,285,277,269,300,389,290,259,288,262,292,308,261,395,325,370,396,297,333,304,371,273,400,378,278,336,305,385,349,280,294,341,316,315,275,391,365,322,328,286,326,342,289,311,335,363,295,353,346,343,296,309,369,319,430,403,323,339,424,381,301,340,293,299,387,447,429,468,475,331,474,344,489,477,306,337,520,469,338,358,345,376,483,321,388,380,350,351,348,347,384,383,374,402,419,516,417,406,368,530,366,571,422,394,545,382,379,440,690,329,390,362,593,392,525,465,412,555,334,413,357,359,375,367,615,377,404,529,749,397,398,498,554,386,619,441,601,354,742,352,446,612,467,372,452,460,393,445,471,457,656,408,827,373,459,470,454,420,401,462,755,500,482,415,553,428,598,487,563,509,521,565,607,405,960,506,624,561,399,476,464,432,479,414,536,463,411,484,834,416,410,427,421,407,425,585,663,433,857,431,673,443,461,418,437,409,480,730,436,448,794,717,435,513,423,466,494,752,458,646,645,634,740,586,835,528,478,438,456,434,451,450,975,594,584,444,973,449,790,517,580,439,473,426,772,628,562,620,640,626,892,650,486,442,534,683,682,621,710,685,660,453,662,687,455,499,568,671,505,495,681,485,688,694,670,504,501,492,691,488,692,712,623,543,546,544,493,978,693,507,508,695,804,539,524,514,743,502,497,527,496,674,732,518,519,511,512,515,541,707,731,540,741,532,643,747,667,675,705,526,728,766,679,491,481,988,644,706,997,696,727,652,625,699,797,552,893,799,510,574,744,590,573,591,769,572,665,533,550,664,559,853,855,916,567,522,654,589,631,709,716,639,503,564,819,547,581,711,537,669,596,829,551,622,759,592,538,560,651,704,523,490,945,764,816,556,641,472,558,800,576,531,735,871,856,784,795,566,822,600,783,770,761,721,535,739,610,583,569,653,548,899,817,575,773,604,808,883,861,549,722,570,577,648,647,737,748,617,659,542,760,895,595,627,587,858,629,698,859,636,792,613,891,676,677,811,798,757,609,702,841,904,678,802,700,703,599,597,655,845,738,680,668,726,734,557,860,684,579,762,932,907,578,642,729,672,1000,718,927,863,864,894,697,611,608,701,632,714,666,602,633,831,939,713,758,614,815,881,814,897,603,605,789,999,896,913,649,952,588,791,724,990,689,637,638,879,949,911,793,616,635,887,745,657,846,750,582,776,968,686,779,780,944,715,812,805,708,661,719,720,925,962,974,832,630,723,606,961,763,828,733,971,751,775,874,736,984,618,746,866,765,753,754,959,781,886,998,756,767,838,796,982,803,900,809,989,786,842,844,777,935,771,934,810,867,943,843,885,820,782,868,725,658,852,955,983,963,931,950,801,957,884,785,875,824,854,869,818,825,888,929,877,862,806,880,922,905,926,788,821,994,882,849,914,787,839,902,979,903,830,920,947,876,878,995,833,996,919,872,807,970,924,940,928,836,778,915,930,981,890,865,917,937,954,938,768,933,993,901,840,921,908,910,967,987,912,873,870,823,848,965,813,918,977,992,850,958,851,909,969,826,941,991,774,972,837,847,906,986,889,936,923,898,964,942,953,948,946,951,956,966,980,976,985 : 1000



==> includes/obfuscated_script.tex <==
\begin{figure*}[!ht]
    \begin{lstlisting}[style=htmlcssjs,caption=Example obfuscated canvas font fingerprinting script., label={lst:sample_fp_script_obfuscated}]
    var _0x2c4a=['\x63\x58\x49\x69','\x42\x6a\x58\x44\x6f\x41\x3d\x3d','\x55\x54\x72\x43\x69\x73\x4f\x77\
    x4f\x38\x4f\x6c\x50\x45\x6e\x43\x6d\x77\x30\x3d','\x49\x38\x4f\x38\x49\x4d\x4f\x42\x77\x70\x72\x44\x6
    e\x41\x3d\x3d','\x77\x35\x54\x43\x73\x42\x56\x51','\x77\x37\x62\x43\x69\x4d\x4f\x38\x77\x34\x68\x4e\x
    54\x67\x67\x66\x46\x73\x4f\x74\x47\x77\x3d\x3d','\x4b\x73\x4f\x68\x4c\x38\x4f\x4c\x77\x70\x37\x44\x6d
    \x48\x73\x3d','\x54\x73\x4b\x49\x59\x43\x64\x64\x77\x35\x4e\x6e\x55\x63\x4b\x31','\x77\x70\x6c\x46\x7
    7\x36\x54\x43\x6e\x38\x4b\x38\x77\x34\x50\x43\x6c\x43\x48\x43\x75\x79\x45\x3d','\x4c\x4d\x4f\x72\x4b\
    x38\x4f\x48\x77\x70\x72\x44\x6b\x56\x76\x44\x73\x42\x76\x44\x6c\x73\x4f\x55\x77\x72\x63\x54','\x77\x3
    5\x44\x44\x73\x56\x76\x43\x74\x4d\x4b\x53'];(function(_0x55d143,_0x164825){var _0x42d32d=function(_0x1
    42de3){while(--_0x142de3){_0x55d143['push'](_0x55d143['shift']());}};var _0x432d6b=function(){var _0x1
    aee5f={'data':{'key':'cookie','value':'timeout'},'setCookie':function(_0x4b8bc7,_0x16461e,_0x593ef0,_0
    x18039c){_0x18039c=_0x18039c||{};var _0x44eb21=_0x16461e+'='+_0x593ef0;var _0x2cd547=0x0;for(var _0x2c
    d547=0x0,_0x253b0d=_0x4b8bc7['length'];_0x2cd547<_0x253b0d;_0x2cd547++){var _0x8355=_0x4b8bc7[_0x2cd54
    7];_0x44eb21+=';\x20'+_0x8355;var _0x471ccc=_0x4b8bc7[_0x8355];_0x4b8bc7['push'](_0x471ccc);_0x253b0d=
    _0x4b8bc7['length'];if(_0x471ccc!==!![]){_0x44eb21+='='+_0x471ccc;}}_0x18039c['cookie']=_0x44eb21;},'r
    emoveCookie':function(){return'dev';},'getCookie':function(_0x3344ca,_0xeafece){_0x3344ca=_0x3344ca||f
    unction(_0x3e8768){return _0x3e8768;};var _0x326c8a=_0x3344ca(new RegExp('(?:^|;\x20)'+_0xeafece['repl
    ace'](/([.$?*|{}()[]\/+^])/g,'$1')+'=([^;]*)'));var _0x43e917=function(_0xc1b2d0,_0x4f4eb4){_0xc1b2d0(
    ++_0x4f4eb4);};_0x43e917(_0x42d32d,_0x164825);return_0x326c8a?decodeURIComponent(_0x326c8a[0x1]):undef
    ined;}};var _0x59f013=function(){var _0x22099e=new RegExp('\x5cw+\x20*\x5c(\x5c)\x20*{\x5cw+\x20*[\x27
    |\x22].+[\x27|\x22];?\x20*}');return_0x22099e['test'](_0x1aee5f['removeCookie']['toString']());};_0x1a
    ee5f['updateCookie']=_0x59f013;var _0x557cbc='';var _0x16beeb=_0x1aee5f['updateCookie']();if(!_0x16bee
    b){_0x1aee5f['setCookie'](['*'],'counter',0x1);}else if(_0x16beeb){_0x557cbc=_0x1aee5f['getCookie'](nu
    ll,'counter');}else{_0x1aee5f['removeCookie']();}};_0x432d6b();}(_0x2c4a,0x10f));var _0x5d52=function(
    _0x30c63c,_0x23c8c2){_0x30c63c=_0x30c63c-0x0;var _0xda86f8=_0x2c4a[_0x30c63c];if(_0x5d52['QtctXq']===u
    ndefined){(function(){var _0x130c23;try{var_0x54738c=Function('return\x20(function()\x20'+'{}.construc
    tor(\x22return\x20this\x22)(\x20)'+');');_0x130c23=_0x54738c();}catch(_0x478721){_0x130c23=window;}var
    _0x443429='ABCDEFGHIJKLMNOPQRSTUVWXYZabcdefghijklmnopqrstuvwxyz0123456789+/=';_0x130c23['atob']||(_0x1
    30c23['atob']=function(_0xd40444){var _0x3d3591=String(_0xd40444)['replace'](/=+$/,'');for(var _0x6f9f
    d2=0x0,_0x52c224,_0x240186,_0x5f4f29=0x0,_0x1a6ef1='';_0x240186=_0x3d3591['charAt'](_0x5f4f29++);~_0x2
    40186&&(_0x52c224=_0x6f9fd2%0x4?_0x52c224*0x40+_0x240186:_0x240186,_0x6f9fd2++%0x4)?_0x1a6ef1+=String[
    'fromCharCode'](0xff&_0x52c224>>(-0x2*_0x6f9fd2&0x6)):0x0){_0x240186=_0x443429['indexOf'](_0x240186);}
    return _0x1a6ef1;});}());var _0x38cf46=function(_0x2b8ed6,_0x23c8c2){var _0x27ff87=[],_0x2b3ad1=0x0,_0
    x1b6fe0,_0x48998d='',_0x214692='';_0x2b8ed6=atob(_0x2b8ed6);for(var_0x17504d=0x0,_0x1b912d=_0x2b8ed6['
    length'];_0x17504d<_0x1b912d;_0x17504d++){_0x214692+='%'+('00'+_0x2b8ed6['charCodeAt'](_0x17504d)['toS
    tring'](0x10))['slice'](-0x2);}_0x2b8ed6=decodeURIComponent(_0x214692);for(var_0x51df8b=0x0;_0x51df8b<
    0x100;_0x51df8b++){_0x27ff87[_0x51df8b]=_0x51df8b;}for(_0x51df8b=0x0;_0x51df8b<0x100;_0x51df8b++){_0x2
    b3ad1=(_0x2b3ad1+_0x27ff87[_0x51df8b]+_0x23c8c2['charCodeAt'](_0x51df8b%_0x23c8c2['length']))%0x100;_0
    x1b6fe0=_0x27ff87[_0x51df8b];_0x27ff87[_0x51df8b]=_0x27ff87[_0x2b3ad1];_0x27ff87[_0x2b3ad1]=_0x1b6fe0;
    }_0x51df8b=0x0;_0x2b3ad1=0x0;for(var _0x1eb95b=0x0;_0x1eb95b<_0x2b8ed6['length'];_0x1eb95b++){_0x51df8
    b=(_0x51df8b+0x1)%0x100;_0x2b3ad1=(_0x2b3ad1+_0x27ff87[_0x51df8b])%0x100;_0x1b6fe0=_0x27ff87[_0x51df8b
    ];_0x27ff87[_0x51df8b]=_0x27ff87[_0x2b3ad1];_0x27ff87[_0x2b3ad1]=_0x1b6fe0;_0x48998d+=String['fromChar
    Code'](_0x2b8ed6['charCodeAt'](_0x1eb95b)^_0x27ff87[(_0x27ff87[_0x51df8b]+_0x27ff87[_0x2b3ad1])%0x100]
    );}return _0x48998d;};_0x5d52['lwrXFx']=_0x38cf46;_0x5d52['UzPXMq']={};_0x5d52['QtctXq']=!![];}var _0x
    4d895c=_0x5d52['UzPXMq'][_0x30c63c];if(_0x4d895c===undefined){if(_0x5d52['kJKNLF']===undefined){var_0x
    2f186f=function(_0x3f061b){this['KdGcrH']=_0x3f061b;this['pFhLAN']=[0x1,0x0,0x0];this['dMSaIq']=functi
    on(){return'newState';};this['EtXeph']='\x5cw+\x20*\x5c(\x5c)\x20*{\x5cw+\x20*';this['ONedVC']='[\x27|
    \x22].+[\x27|\x22];?\x20*}';};_0x2f186f['prototype']['CZgCEj']=function(){var _0x3b1467=new RegExp(thi
    s['EtXeph']+this['ONedVC']);var _0x5270d0=_0x3b1467['test'](this['dMSaIq']['toString']())?--this['pFhL
    AN'][0x1]:--this['pFhLAN'][0x0];return this['UekVUm'](_0x5270d0);};_0x2f186f['prototype']['UekVUm']=fu
    nction(_0x2669eb){if(!Boolean(~_0x2669eb)){return _0x2669eb;}return this['VCeZON'](this['KdGcrH']);};_
    0x2f186f['prototype']['VCeZON']=function(_0x144334){for(var_0x1e4db6=0x0,_0x3d036c=this['pFhLAN']['len
    gth'];_0x1e4db6<_0x3d036c;_0x1e4db6++){this['pFhLAN']['push'](Math['round'](Math['random']()));_0x3d03
    6c=this['pFhLAN']['length'];}return _0x144334(this['pFhLAN'][0x0]);};new_0x2f186f(_0x5d52)['CZgCEj']()
    ;_0x5d52['kJKNLF']=!![];}_0xda86f8=_0x5d52['lwrXFx'](_0xda86f8,_0x23c8c2);_0x5d52['UzPXMq'][_0x30c63c]
    =_0xda86f8;}else{_0xda86f8=_0x4d895c;}return _0xda86f8;}webg;var _0x364fa4=function(){var _0x172ba0=!!
    [];return function(_0x47a250,_0x18c49a){var _0x5111d9=_0x172ba0?function(){if(_0x18c49a){var _0x3d31bb
    =_0x18c49a['apply'](_0x47a250,arguments);_0x18c49a=null;return _0x3d31bb;}}:function(){};_0x172ba0=![]
    ;return _0x5111d9;};}();var _0xbe7379=_0x364fa4(this,function(){var _0x35f6e2=function(){return'\x64\x
    65\x76';},_0x4c1c29=function(){return'\x77\x69\x6e\x64\x6f\x77';};var _0x311e1d=function(){var _0x4030
    fb=newRegExp('\x5c\x77\x2b\x20\x2a\x5c\x28\x5c\x29\x20\x2a\x7b\x5c\x77\x2b\x20\x2a\x5b\x27\x7c\x22\x5d
    \x2e\x2b\x5b\x27\x7c\x22\x5d\x3b\x3f\x20\x2a\x7d');return!_0x4030fb['\x74\x65\x73\x74'](_0x35f6e2['\x7
    4\x6f\x53\x74\x72\x69\x6e\x67']());};var _0x3b02d1=function(){var _0x486df3=new RegExp('\x28\x5c\x5c\x
    5b\x78\x7c\x75\x5d\x28\x5c\x77\x29\x7b\x32\x2c\x34\x7d\x29\x2b');return _0x486df3['\x74\x65\x73\x74'](
    _0x4c1c29['\x74\x6f\x53\x74\x72\x69\x6e\x67']());};var _0x466dea=function(_0x3aeaa3){var _0x575475=~-0
    x1>>0x1+0xff%0x0;if(_0x3aeaa3['\x69\x6e\x64\x65\x78\x4f\x66']('\x69'===_0x575475)){_0xcc14f2(_0x3aeaa3
    );}};var _0xcc14f2=function(_0x2c171b){var _0x20a62f=~-0x4>>0x1+0xff%0x0;if(_0x2c171b['\x69\x6e\x64\x6
    5\x78\x4f\x66']((!![]+'')[0x3])!==_0x20a62f){_0x466dea(_0x2c171b);}};if(!_0x311e1d()){if(!_0x3b02d1())
    {_0x466dea('\x69\x6e\x64\u0435\x78\x4f\x66');}else{_0x466dea('\x69\x6e\x64\x65\x78\x4f\x66');}}else{_0
    x466dea('\x69\x6e\x64\u0435\x78\x4f\x66');}});_0xbe7379();var _0x1b2b65=[_0x5d52('0x0','\x62\x5d\x75\x
    41'),_0x5d52('0x1','\x69\x28\x46\x25')];var _0x1d1d56=document[_0x5d52('0x2','\x28\x6d\x68\x26')]('\x6
    3\x61\x6e\x76\x61\x73');_0x1d1d56[_0x5d52('0x3','\x65\x23\x25\x7a')]=_0x5d52('0x4','\x28\x4d\x43\x54')
    ;_0x1d1d56['\x68\x65\x69\x67\x68\x74']=_0x5d52('0x5','\x54\x52\x53\x4b');var _0x4d24cc=_0x1d1d56[_0x5d
    52('0x6','\x44\x78\x34\x5b')]('\x32\x64');var _0x3284af={};for(i=0x0;i<_0x1b2b65[_0x5d52('0x7','\x28\x
    6d\x68\x26')];i++){_0x1d1d56[_0x5d52('0x8','\x67\x33\x48\x21')]=_0x1b2b65[i];_0x3284af[_0x1b2b65[i]]=_
    0x4d24cc[_0x5d52('0x9','\x35\x70\x64\x4c')](_0x5d52('0xa','\x28\x6d\x68\x26'))['\x77\x69\x64\x74\x68'];}
    \end{lstlisting}
    \end{figure*}
    
